Gripper Keypose and Object Pointflow as Interfaces for Bimanual Robotic Manipulation

Bimanual manipulation is a challenging yet crucial robotic capability, demanding precise spatial localization and versatile motion trajectories, which pose significant challenges to existing approaches. Existing approaches fall into two categories: keyframe-based strategies, which predict gripper poses in keyframes and execute them via motion planners, and continuous control methods, which estimate actions sequentially at each timestep. The keyframe-based method lacks inter-frame supervision, struggling to perform consistently or execute curved motions, while the continuous method suffers from weaker spatial perception. To address these issues, this paper introduces an end-to-end framework PPI (keyPose and Pointflow Interface), which integrates the prediction of target gripper poses and object pointflow with the continuous actions estimation. These interfaces enable the model to effectively attend to the target manipulation area, while the overall framework guides diverse and collision-free trajectories. By combining interface predictions with continuous actions estimation, PPI demonstrates superior performance in diverse bimanual manipulation tasks, providing enhanced spatial localization and satisfying flexibility in handling movement restrictions. In extensive evaluations, PPI significantly outperforms prior methods in both simulated and real-world experiments, achieving state-of-the-art performance with a +16.1% improvement on the RLBench2 simulation benchmark and an average of +27.5% gain across four challenging real-world tasks. Notably, PPI exhibits strong stability, high precision, and remarkable generalization capabilities in real-world scenarios. Project page: https://yuyinyang3y.github.io/PPI/

==> rebuttal_tables/improved_and_new_tasks.tex <==
\begin{tabular}{lcccccc}
\toprule
\multirow{2}{*}{Method} 
& \multicolumn{3}{c}{Improved Baseline} 
& \multicolumn{3}{c}{New Tasks in Real-World} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7}
& Carry the Tray
& Handover \& Insert the Plate
& Wipe the Plate
& Wear the Scarf
& Press the Cap of Bottle
& Scan the Bottle (Unimanual)\\
\midrule \midrule 
ACT 
& 30.0 / 30.0 / 5.5
& 10.0 / 70.0 / 5.5
& 0.00 / 40.0 / 3.8
& 40.0 / 70.0 / 5.7
& 10.0 / 20.0 / 3.0
& 20.0 / 70.0 / 4.7
\\
% 
DP3
& 50.0 / 50.0 / 6.0
& 20.0 / 80.0 / 4.7
& 40.0 / 60.0 / 6.5
& /
& /
& /
\\
%
Ours (simple 10Hz)
& 50.0 / 70.0 / 6.0
& 30.0 / 100 / 5.7
& 50.0 / 70.0 / 6.8
& /
& /
& /
\\
%
\baseline{Ours (2.5Hz)} 
& \baseline{\textbf{50.0} / \textbf{100} / \textbf{7.5}}
& \baseline{\textbf{40.0} / \textbf{100} / \textbf{7.7}}
& \baseline{\textbf{70.0} / \textbf{70.0} / \textbf{8.3}}
& \baseline{\textbf{70.0} / \textbf{80.0} / \textbf{7.7}}
& \baseline{\textbf{40.0} / \textbf{80.0} / \textbf{6.7}}
& \baseline{\textbf{80.0} / \textbf{100} / \textbf{9.3}}
\\
\bottomrule
\end{tabular}

==> rebuttal_tables/improved_and_simple.tex <==
\begin{tabular}{cccc}
\toprule
\multirow{2}{*}{Method} & 
\multicolumn{3}{c}{SR (\%) $\uparrow$ /Loc-SR (\%) $\uparrow$ / Normalized Score $\uparrow$} \\
\cline{2-4}
& Carry the Tray
& Handover \& Insert the Plate
& Wipe the Plate
\\
\midrule \midrule 
ACT 
& 30.0 / 30.0 / 5.5
& 10.0 / 70.0 / 5.5
& 0.00 / 40.0 / 3.8
\\
% 
DP3
& 50.0 / 50.0 / 6.0
& 20.0 / 80.0 / 4.7
& 40.0 / 60.0 / 6.5
\\
%
Ours Simple (10.52 Hz)
& 50.0 / 70.0 / 6.0
& 30.0 / 100 / 5.7
& 50.0 / 70.0 / 6.8
\\
%
\baseline{Ours (2.63 Hz)} 
& \baseline{\textbf{50.0} / \textbf{100} / \textbf{7.5}}
& \baseline{\textbf{40.0} / \textbf{100} / \textbf{7.7}}
& \baseline{\textbf{70.0} / \textbf{70.0} / \textbf{8.3}}
\\
\bottomrule
\end{tabular}

==> rebuttal_tables/kfnum_ablation.tex <==
\begin{tabular}{cccccccccc}
\toprule
% \multicolumn{1}{c}{\multirow{3}{*}{Method}} & 
% \multicolumn{1}{c}{\multirow{3}{*}{{Avg. Success $\uparrow$ }} } & 
Keyframe Type & Avg. KF Nums & Avg. SR(\%) $\uparrow$ & Box(\%) & Ball(\%) &  Drawer(\%)  & Laptop(\%)  &  Dustpan(\%) & Tray(\%)   & Handover Easy(\%)  \\
\midrule \midrule 
% last timestep & 1 & 69.8  & 88 & 81 & 25  & \textbf{58} & 99 & 92& 46  \\
gripper openness & 2.7 & 64.9  & 88 & 81 & 30 & 35 & 99& 82& 39\\

% \midrule \midrule
% continuous on pointflow & 70.0 
% & 89.3 \textcolor{grey!50}{\tiny$\pm 4.6$} 
% & 62.0 \textcolor{grey!50}{\tiny$\pm 13.0$} 
% & 80.0 \textcolor{grey!50}{\tiny$\pm 6.1$}
% & 22.0 \textcolor{grey!50}{\tiny $\pm 6.3$}
% & 99.0 \textcolor{grey!50}{\tiny$\pm 0.0$} 
% & 90.7 \textcolor{grey!50}{\tiny$\pm 1.5$} 
% & 47.2\textcolor{grey!50}{\tiny$\pm 3.0$}\\
\baseline{Ours (Best Ckpt)} & \baseline{10} & \baseline{\textbf{82.6}}
& \baseline{\textbf{98}}
& \baseline{\textbf{91}}
& \baseline{\textbf{84}}
& \baseline{\textbf{47}}
& \baseline{\textbf{100}}
& \baseline{\textbf{93}}
& \baseline{\textbf{65}} \\
% \baseline{Ours (Averaged)} & \baseline{80.8}
% & \baseline{96.7}
% & \baseline{89.3}
% & \baseline{79.7}
% & \baseline{46.3}
% & \baseline{98.7}
% & \baseline{92.0}
% & \baseline{62.7} \\
\bottomrule
\end{tabular}

==> rebuttal_tables/sim_tasks.tex <==
\begin{tabular}{cccccccccc}
\toprule
% \multicolumn{1}{c}{\multirow{3}{*}{Method}} & 
% \multicolumn{1}{c}{\multirow{3}{*}{{Avg. Success $\uparrow$ }} } & 
Method 
& Handover Item(\%) 
& Put Bottle in Fridge(\%)  \\
\midrule \midrule 
ACT 
&  0
&  0
\\
% 
PerAct$^2$ 
&  11
&  3
\\
3D Diffuser Actor 
& 19
& 38
\\
% 
\baseline{Ours} 
& \baseline{\textbf{56}}
& \baseline{\textbf{92}}
\\
\bottomrule
\end{tabular}
